Online Algorithms with Multiple Predictions

This paper studies online algorithms augmented with multiple machine-learned predictions. While online algorithms augmented with a single prediction have been extensively studied in recent years, the literature for the multiple predictions setting is sparse. In this paper, we give a generic algorithmic framework for online covering problems with multiple predictions that obtains an online solution that is competitive against the performance of the best predictor. Our algorithm incorporates the use of predictions in the classic potential-based analysis of online algorithms. We apply our algorithmic framework to solve classical problems such as online set cover, (weighted) caching, and online facility location in the multiple predictions setting. Our algorithm can also be robustified, i.e., the algorithm can be simultaneously made competitive against the best prediction and the performance of the best online algorithm (without prediction).

==> facility-old.tex <==
We now apply our framework to the online \fac problem. We first describe the offline version of this problem. An instance of \fac is given by a metric space $d(\cdot, \cdot)$,  a set of $m$ potential facility location points $\cal F$, and a set $\cal R$ of clients in the  metric space. 
Further, each location $f_j \in {\cal F}$ has a facility opening cost $o_j$. 
vA solution opens a subset ${\cal F}' \subseteq {\cal F}$ of facilities, and assigns each client $r_i$ to the closest open facility $f_{j_i} \in {\cal F}'$. The connection cost of this client is $d(r_j, f_{j_i})$ and the goal is to minimize the sum of the connection costs of all the clients and the facility opening costs of the facilities in ${\cal F}'.$

We now describe the natural LP relaxation for \fac; our notion of a fractional solution will be with respect to this LP relaxation. 
We have variables $y_j$ for each facility location $f_j \in {\cal F
}$, which denotes the extent to which facility $j$ is open, and variables $x_{ij}$ for each client $r_i$ and facility $f_j$ denoting the extent to which $r_i$ is assigned to $f_j$. The relaxation is as follows:

\begin{align}
\text{Minimize } \sum_{j=1}^m o_j y_j & + \sum_{i=1}^{n}\sum_{j=1}^{m} d_{ij} x_{ij} \text{ subject to} \nonumber\\
   x_{ij} &\leq y_{j} \quad \forall i, j \label{eq:fac1}\\
   \sum_{j=1}^{m}x_{ij} &= 1 \quad \forall i \label{eq:fac2} \\
    y_j &\in [0, 1] \quad \forall j
\end{align}

In the online \fac problem, clients arrive over time and the solution needs to assign each arriving client to an open facility. The algorithm can also open facilities at any time. We now consider online \fac in the multiple predictions setting. Before describing the algorithm, we formalize the problem. 
 At each step $i$,  a client request $r_i$ arrives and we are given $k$ predictions, $S_1, S_2, \ldots S_{k}$, where each prediction $S_\ell$ is given by the fractional values $ \{(y_{1\ell}, y_{2\ell}, \ldots y_{m\ell}), (x_{i,1, \ell}, x_{i,2,\ell}, \ldots x_{i,m, \ell})\}$ such that $y_{j\ell}$ is the suggested value  for $y_{j}$ and $x_{i, j, \ell}$ is the suggested value for $x_{ij}$. These values ensure that the constraints~\eqref{eq:fac1} and~\eqref{eq:fac2} are satisfied for the client $r_i$. 
 As before, the online algorithm must maintain a feasible fractional solution to satisfy the constraints in the LP relaxation.

\subsection{Online Algorithm}

The algorithm is described in~\Cref{alg: Dynamic_OPT_fac_loc}. As earlier, 
%we raise a time variable $t$ uniformly and 
for all $j$, we simultaneously raise $x_{ij}$ (and possibly $y_j$ as well) at the rate specified by the algorithm. As in the case of online covering problem, we raise these variables only till the client $r_i$ is satisfied to an extent of at least $1/2$. In the actual algorithm, we will double these variables so that each arriving client is satisfied to an extent of 1. 


\begin{algorithm}[H]
\caption{Algorithm for Online \fac}
\label{alg: Dynamic_OPT_fac_loc}
On arrival of the client $r_i$: \\
\hspace*{20pt} \textbf{Initialize} $x_{ij} = 0, \quad \forall j$. \\
\hspace*{20pt} \textbf{Initialize} $\Gamma_{ij} := \sum_{\ell=1}^{k}x_{i,j,\ell}, \quad \forall j$. \\
\hspace*{50pt} \textbf{While $\sum_j x_{ij} < \frac{1}{2}$}  \\
\hspace*{80pt} \textbf{For all} $j$: \\
\hspace*{100pt} \textbf{If} $x_{ij} < y_j$ \\
\hspace*{120pt} Increase  $x_{ij}$ at the rate $\frac{d x_{ij}}{d t} = \left(\frac{1}{d_{ij}}\right)\cdot\left(x_{ij} + \frac{\Gamma_{ij}}{k}\right) $ \\
\hspace*{100pt} \textbf{Else} \\
\hspace*{120pt} Increase both variables $x_{ij}, y_{j}$ at the same rate \\
\hspace*{130pt} $\frac{d y_{j}}{d t} = \frac{d x_{ij}}{d t} = \left(\frac{1}{d_{ij}+o_j}\right)\cdot\left(x_{ij} + \frac{\Gamma_{ij}}{k}\right) $.\\
\end{algorithm}



\subsection{Analysis}
In this section, we analyze~\Cref{alg: Dynamic_OPT_fac_loc}. Fix an index $i$, and consider the input till step $i$. Let $x^\opt, y^\opt$ be the best dynamic solution till this step.  We first bound the rate of increase of the cost of the algorithm. 
\begin{lemma}
\label{lem:costfac}
The rate of increase of the cost for~\Cref{alg: Dynamic_OPT_fac_loc} is at most $\frac32$.
\end{lemma}
\begin{proof}
For any fixed $j$, we claim:
\begin{align}
    \label{eq:proof1}
    d_{ij}\cdot \frac{\partial x_{ij}}{\partial t}+ o_{j}\cdot \frac{\partial y_{j}}{\partial t} =
    x_{ij} + \frac{\Gamma_{ij}}{k}. 
\end{align}
To show this, there are two cases to consider:
\begin{itemize}
    \item $x_{ij} < y_j$: In this case, $\frac{\partial y_{ij}}{\partial t} = 0$, and  $d_{ij}\cdot \frac{\partial x_{ij}}{\partial t} = x_{ij} + \frac{\Gamma_{ij}}{k}$m and so~\eqref{eq:proof1} holds. 
    \item $x_{ij} = y_j$: In this case, $\frac{\partial y_{ij}}{\partial t} = \frac{\partial x_{ij}}{\partial t} = \frac{x_{ij} + \frac{\Gamma_{ij}}{k}}{d_{ij}+o_j}$, i.e.,
    $o_j\cdot \frac{\partial y_{ij}}{\partial t} + d_{ij}\cdot \frac{\partial x_{ij}}{\partial t} = x_{ij} + \frac{\Gamma_{ij}}{k}$,
    and so~\eqref{eq:proof1} holds. 
\end{itemize}
%
Therefore, the rate of change of the objective function is given by:
\[
    \sum_{j}\left(d_{ij}\cdot \frac{\partial x_{ij}}{\partial t}+ o_{j}\cdot \frac{\partial y_{j} }{\partial t}\right) 
    \stackrel{\eqref{eq:proof1}}{=} \sum_{j}\left(x_{ij} + \frac{\Gamma_{ij}}{k}\right) 
    = \sum_{j}x_{ij} + \frac{\sum_{\ell} \sum_{j} x_{i,j,\ell}}{k}
    \le \frac12 + 1
    = \frac32.\qedhere
\]
\end{proof}


We now describe the potential function, which has a similar structure as that in the online covering framework. 
Let $\xd_{ij}, \yd_j$ denote the values of the variables $x_{ij}, y_j$ respectively in the benchmark solution $\dynamic$. The potential function for a variable $x_{ij}$ is then  as follows:
\[
    \phi_{ij} = d_{ij} \cdot \xd_{ij} \cdot \ln \frac{(1+\delta) \xd_{ij}}{x_{ij} + \delta \xd_{ij}}, \text{ where } \delta = 1/k,
\]
and the potential for the variable $y_j$ is given by 
$$  \psi_{j} = o_j \cdot \yd_{j} \cdot \ln \frac{(1+\delta) \yd_{j}}{y_{j} + \delta \yd_{j}}.$$
%
As before, the overall potential is 
\[
    \phi = \sum_{i,j: \xd_{ij}\ge x_{ij}} \phi_{ij} +\sum_{j: \yd_{j}\ge y_{j}} \psi_{j} .
\]
%
The rest of the proof proceeds along the same lines as that for the online covering problem. But we give the details for the sake of completeness.

The next lemma is the analogue of~\Cref{lem:pot-nonneg}, and shows that the potential $\phi$ is always non-negative. 
\begin{lemma}
\label{lem:pot-nonneg1}
    For any values of the variables $x_{ij},y_j, , \xd_{ij}, \yd_j$, the potential function $\phi$ is non-negative.
\end{lemma}
\begin{proof}
We show that each of the quantities $\phi_{ij}, \psi_j$ in the expression for $\phi$ is non-negative. Consider a pair $i,j$ for which $\xd_{ij} \geq x_{ij}$. Then
       $$ \phi_{ij} = d_{ij} \cdot \xd_{ij} \cdot \ln \frac{(1+\delta) \xd_{ij}}{x_{ij} + \delta \xd_{ij}} 
        = d_{ij} \cdot \xd_{ij} \cdot \ln \frac{1+\delta}{\frac{x_{ij}}{\xd_{ij}} + \delta} \ge 0.
    $$
    Similarly, $\psi_j \geq 0$ if $\yd_j \geq y_j$. This shows that $\phi \geq 0$. 
    \qedhere
\end{proof}

Now we bound the potential against the benchmark solution \dynamic. The proof of this lemma is very similar to that of~\Cref{lem:opt-pot}. 

\begin{lemma}
\label{lem:opt-pot1}
    The following bounds hold: $\phi_{ij} \le d_{ij}\cdot  \ln (1+\frac{1}{\delta}) = d_{ij}\cdot O(\log k)$ and $\psi_{j} \le o_{j} \cdot \ln (1+\frac{1}{\delta})) = o_{j}\cdot O(\log k)$. As a consequence, the overall potential $\phi \le O(\log k)\cdot \left(\sum_i \sum_j d_{ij} \xd_{ij} + \sum_j o_j \yd_j\right)$.
\end{lemma}
\begin{proof}
We have 
\[
    \phi_{ij} 
    = d_{ij} \xd_{ij} \cdot \ln \frac{(1+\delta) \xd_{ij}}{x_i + \delta \xd_{ij}}
    \le d_{ij} \xd_{ij} \cdot \ln \frac{(1+\delta) \xd_{ij}}{\delta \xd_{ij}}
    = d_{ij} \xd_{ij} \cdot \ln \left(1+\frac{1}{\delta}\right)
    = d_{ij} \xd_{ij} \cdot O(\log k).
\]    
The bound for $\psi_j$ also follows similarly.
\end{proof}

Finally, we bound the rate of decrease of potential $\phi$ with increase in the variables in \Cref{alg: Dynamic_OPT_fac_loc}. 
\begin{lemma}
\label{lem:alg-pot1} 
    The rate of decrease of the potential $\phi$ in \Cref{alg: Dynamic_OPT_fac_loc} is at least $\frac12$.
\end{lemma}
\begin{proof}
It is easy to check that 
\begin{equation}\label{eq:phix1}
    \frac{\partial \phi_{ij}}{\partial x_{ij}} = - d_{ij}\cdot \frac{\xd_{ij}}{x_{ij}+\delta \xd_{ij}}, \quad \frac{\partial \psi_{j}}{\partial y_{j}} = - o_{j}\cdot \frac{\yd_{j}}{y_{j}+\delta \yd_{j}}.
\end{equation}

Consider the step when the client request $r_i$ arrives. We claim that for any index $j \in [m]$, 
\begin{align}
    \label{eq:phix2}
    \frac{d \left( \phi_{ij} + \psi_j \right)}{dt} \leq - \xd_{ij} \cdot \frac{x_{ij} + \delta \Gamma_{ij}}{x_{ij} + \delta \xd_{ij}}.
\end{align}

To prove this, we consider two cases: 
\begin{itemize}
    \item $x_{ij} < y_j$: In this case, $\frac{d x_{ij}}{dt} = \frac{1}{d_{ij}} \cdot \left( x_{ij} + \frac{\Gamma_{ij}}{k} \right), \frac{dy_j}{dt} = 0$. Combining this with~\eqref{eq:phix1}, we see that 
    $$ \frac{d \left( \phi_{ij} + \psi_j \right)}{dt} = \frac{d \phi_{ij}}{dt} = \frac{d \phi_{ij}}{dx_{ij}} \cdot \frac{d x_{ij}}{dt} = -\xd_{ij} \cdot 
    \frac{x_{ij} + \delta \Gamma_{ij}}{x_{ij} + \delta \xd_{ij}}.$$
    \item $x_{ij} = y_j$: In this case, $\frac{d x_{ij}}{dt} = \frac{dy_j}{dt} = \frac{1}{d_{ij}+o_j} \cdot \left( x_{ij} + \frac{\Gamma_{ij}}{k} \right). $
    Using~\eqref{eq:phix1} again and the fact that $y_j = x_{ij}$, we see that 
    $$ \frac{d \left( \phi_{ij} + \psi_j \right)}{dt} = \frac{d \phi_{ij}}{d x_{ij}} \cdot \frac{dx_{ij}}{dt} + \frac{d \psi_j}{d y_j} \cdot \frac{dy_j}{dt} = - \frac{1}{o_j + d_{ij}} \left( \frac{d_{ij} \xd_{ij}}{x_{ij} + \delta \xd_{ij}} + \frac{o_j \yd_j}{x_{ij} + \delta \yd_j}\right)  \cdot  \left( x_{ij} + \delta \Gamma_{ij} \right).$$
    Since $\yd_j \geq \xd_{ij}, \frac{\yd_j}{x_{ij} + \delta \yd_j} \geq \frac{\xd_{ij}}{x_{ij} + \delta \xd_{ij}}.$
Therefore, the RHS above is at most $ - \xd_{ij} \cdot \frac{x_{ij} + \delta \Gamma_{ij}}{x_{ij} + \delta \xd_{ij}}.$    
\end{itemize}

Thus, we have shown that inequality~\eqref{eq:phix2} always holds. 
Now, we have two cases:
\begin{itemize}
    \item  $\Gamma_{ij} \ge \xd_{ij}$: Inequality~\eqref{eq:phix2} implies that 
    \[
        \frac{d (\phi_{ij}+ \psi_j)}{dt} \le -\xd_{ij}.
    \]
    \item $\Gamma_{ij} < \xd_{ij}$: Using~\eqref{eq:phix2} again, we see that 
    \[
        \frac{d (\phi_{ij}+\psi_j)}{dt} 
        \leq - \cdot \xd_{ij} \cdot \frac{x_{ij} + \delta\cdot \Gamma_{ij}}{x_{ij} + \delta \xd_{ij}}
        = - \cdot \Gamma_{ij}\cdot \frac{\frac{\xd_{ij}}{\Gamma_{ij}}\cdot x_{ij} + \delta\cdot \xd_{ij}}{x_{ij} + \delta \xd_{ij}}
        \leq - \Gamma_{ij}.
    \]
\end{itemize}
We know that at least one of the suggestions in the $i$-th step is supported by the \dynamic benchmark. Let $\ell_i \in [k]$ be the index of such a supported suggestion. Then,
\begin{align*}
    \Gamma_{ij} &= \sum_{\ell=1}^k x_{ij\ell} \geq x_{ij\ell_i}, \text{ and }\\
    \xd_{ij} &\ge x_{ij \ell_i} \text{ since } \ell_i \text{ is supported by \dynamic}.
\end{align*}
Therefore, in both cases above, we get
\[
    \frac{d(\phi_{ij}+ \psi_j)}{dt} \le - x_{ij\ell_i}.
\]

\noindent
Let $J$ denote the index set $\{j: \xd_{ij} \geq x_{ij}\}$. 
We claim that the 
total decrease in potential satisfies:
\begin{align}
\label{eq:decpot}
    \frac{d\Phi}{dt} \leq -\sum_{j \in J} x_{ij\ell_i}.
\end{align}
To see this, let $J'$ denote the index set $\{j: \yd_j \geq y_j \}$. Then the term in $\phi$ corresponding to step $i$ is $\phi_i := \sum_{j \in J} \phi_{ij} + \sum_{j \in J'} \psi_j. $ First consider an index $j \in J$ for which $x_{ij} < y_j$. In this case, we know that $\frac{d \psi_j}{dt} = 0$, and so irrespective of whether $j$ belongs to $J'$ or not, the rate of change of the terms in $\phi_i$ corresponding to $j$ is 
$$ \frac{d(\phi_{ij} + \psi_j)}{dt} \leq -x_{ij \ell_i}. $$ Now consider an index $j \in J$ for which $x_{ij} = y_j$. Since $\yd_j \geq \xd_{ij}$, it follows that $\yd_j \geq y_j$ and so $j \in J'$ as well. Therefore, the rate of change of the terms in $\phi_i$ corresponding to $j$ is equal to 
$$\frac{d(\phi_{ij} + \psi_j)}{dt} \leq -x_{ij \ell_i}. $$
Finally, consider an index $j \in J' \setminus J$. It is easy to verify that $\frac{d \psi_j}{dt} \leq 0$. Thus, the inequality~\eqref{eq:decpot} follows. 


The rest of the argument proceeds as in the proof of~\Cref{lem:alg-pot}.
By feasibility of the $l_i$-th suggestion in step $i$, we have:
\begin{align*}
    \sum_j  x_{ij\ell_i} &\ge 1\\
    \text{i.e., } \sum_{j \in J} x_{ij \ell_i} + \sum_{j \notin J} x_{ij\ell_i} &\ge 1\\
    \text{i.e., } \sum_{j \in J} x_{ij \ell_i} + \sum_{j \notin J} x_{ij} &\ge 1 \quad \quad \text{(since } j \notin J \implies x_{ij} \geq \xd_{ij} \geq x_{ij\ell_i})\\
     \text{i.e., } \sum_{j \in J} x_{ij \ell_i} + \sum_{j} x_{ij} &\ge 1 \\
     \text{i.e., } \sum_{j \in J} x_{ij \ell_i}  &\ge \frac12.
\end{align*}
The last step is from the fact the \Cref{alg: Dynamic_OPT_fac_loc} is used only when $\sum_j x_{ij} < 1/2$. The desired result now follows from~\eqref{eq:decpot}. 
\end{proof}
%\alert{OLD POTENTIAL FUNCTION BELOW}
%

%We now lower bound the cost of the best dynamic solution. 

%\begin{lemma}\label{lemma: bound_over_x}
%Let $M' \subseteq [m]$ be the index set defined by $\{j: x_{ij} \le 2\cdot %x^\opt_{ij}\}$. Then we have:
%\begin{equation*}
%    \sum_{j\in M'}x^\opt_{ij} \ge \frac{1}{2}.
%\end{equation*}
%
%\begin{proof} We have
%\begin{align*}
%    1 &= \sum_{j \in M}x^{OPT}_{ij} 
%    \le\sum_{j\in M'} x^{\opt}_{ij} + \frac{1}{2}\cdot\sum_{j \notin M'}x_{ij}\\
%    &\le \sum_{j\in M'}x^{\opt}_{ij}+ \frac{1}{2}\sum_{j}x_{ij}\\
%    &\le \sum_{j\in M'}x^{\opt}_{ij} + \frac{1}{2},
%\end{align*}
%where the second last inequality follows from the fact that $\sum_j x_{ij} = 1$. 
%The above yields $\sum_{j\in M'}x^{\opt}_{ij} \ge \frac{1}{2}$.
%\end{proof}
%\end{lemma}
%
%We are now ready to define the potential function. We give some notation first. We %define the truncated variables $\bar{x}_{ij} = \min\{x_{ij}, 2\cdot x^{OPT}_{ij}\}$, and $\bar{y}_{j,s} = \min\{y_{j}, \frac{2^{s+1}}{m} \}$, where $s$ can be any integer. Now define 
%$$ \phi_{ij} := d_{ij}\cdot x^{\opt}_{ij}\cdot \log \left(\frac{x^{\opt}_{ij}\cdot(2+\frac{1}{k})}{{\bar x}_{ij} + \frac{x^{\opt}_{ij}}{k}}\right),$$
%and 
%$$ \psi_{js} := \left \{ \begin{array}{ll} o_{j}\cdot \frac{2^{s}}{m}\log %\left(\frac{(1+\frac{1}{4k})\cdot\frac{2^{s+1}}{m}}{\bar{y}_{j,s} + %\frac{2^{s-1}}{mk}}\right) & \mbox{ if $y^{\opt}_{j} \ge \frac{2^{s-1}}{m}$} \\
%0 & \mbox{otherwise} \end{array} \right. $$
%
%Finally, define the potential $\Phi$ as 
%$$ \Phi := \sum_{i,j} \phi_{ij} + \sum_{j,s} \psi_{j,s}. $$
%
%
%
%\begin{lemma}\label{lemma:pot_bound}
%The potential $\Phi$ is non-negative and is at most  $4  \log (4k+1) \cdot  C_\opt$.
%\end{lemma}
%\begin{proof}
%Since $\bar{x}_{ij} \leq 2x^\opt_{ij},$ it follows that $\phi_{ij} \geq 0$. Similarly, the fact  that $\bar{y}_{j,s} \leq \frac{2^{s+1}}{m}$ implies that $\psi_{js} \geq 0$. This shows that $\Phi \geq 0$. 
%
%Now we upper bound $\Phi$. Since $\bar{x}_{ij} \geq 0$, it follows that
%\begin{align}
%    \label{eq:xij}
%    \phi_{ij} \leq d_{ij} \cdot x^\opt_{ij} \cdot \log(2k+1). 
%\end{align}
%
%Similarly, for a fixed $j$, let $s_j$ be the integer for which 
%$y^\opt_{j} \in [\frac{2^{s_j}-1}{m}, \frac{2^{s_j}}{m})$. 
%Since $\bar{y}_{js} \geq 0$, it follows that 
%$$ \psi_{js} \leq  \left \{ \begin{array}{ll} o_j \cdot \frac{2^s}{m} \log(4k+1)  & %\mbox{ if $s \leq s_j$} \\
%0 & \mbox{otherwise} \end{array} \right. $$
%
% Hence, we get:
%
%\begin{align}
%\label{eq:yj}
%\sum_{s}\phi_{js} \leq \log(4k+1) \cdot o_j \cdot \sum_{s \leq s_j} \frac{2^s}{m} \leq %4 \log(4k+1) \cdot o_j \cdot y^\opt_j.
%\end{align}
%
%It follows from~\eqref{eq:xij} and~\eqref{eq:yj} that $\Phi \leq 4 \log(4k+1) \cdot %C_\opt. $
%\end{proof}
%
%Recall from the statement of~\Cref{lemma: bound_over_x} that $M'$ is the  set of indices $j$ for which $x_{ij} \leq 2x^\opt_{ij}$. 
%\begin{lemma}\label{lemma: dec_pot_part1}
%Let $j \in M'$. Then, 
%\begin{equation*}
%\frac{\partial \phi_{ij}}{\partial t} + \sum_{s}\frac{\partial \psi_{j,s}}{\partial t} %\le -x^{\opt}_{ij}.
%\end{equation*}
%\end{lemma}
%\begin{proof}
%Since  $x_{ij}\le 2\cdot x^\opt_{ij}$, we get $\bar{x}_{ij} = x_{ij}$. Two cases %arise:
%\begin{itemize}
%    \item $x_{ij} < y_{j}$: In this case $\frac{\partial y_j}{\partial t} = 0$, and so %$\frac{\partial \psi_{js}}{\partial t} = 0$ for all $s$. Therefore, 
%    \begin{align*}
%    \frac{\partial \phi_{ij}}{\partial t} + \sum_{s}\frac{\partial %\psi_{j,s}}{\partial t} &= \frac{\partial \phi_{ij}}{\partial t}
%    =d_{ij}\cdot x^{\opt}_{ij}\cdot \frac{\frac{\partial x_{ij}}{\partial t}}{x_{ij} + %\frac{x^{\opt}_{ij}}{k} }\\
%    &=-x^{\opt}_{ij} \cdot \left(\frac{x_{ij} + \frac{\Gamma_{ij}}{k}}{x_{ij} + %\frac{x^{\opt}_{ij}}{k}}\right)
%    \le -x^{\opt}_{ij},
%\end{align*}
%where the last inequality follows from the fact that $\Gamma_{ij} \geq x^\opt_{ij}$. 
%\end{itemize} 
%
%
%\item $x_{ij}=y_j$:  In this case, we have $\frac{\partial y_j}{\partial t} = %\frac{\partial x_{ij}}{\partial t} = \frac{1}{o_{j} + d_{ij}}\cdot (x_{ij} + %\frac{\Gamma_{ij}}{k})$. Let $s$ be the index for which  $x^{\opt}_{ij} \in %[\frac{2^{s_j-1}}{m}, \frac{2^{s_j}}{m}]$. It is easy to check that Then, 
%\begin{align*}
 %   \frac{\partial \phi_{ij}}{\partial t} + \sum_{s}\frac{\partial %\psi_{j,s}}{\partial t} &\le  \frac{\partial \phi_{ij}}{\partial t} + \frac{\partial %\psi_{j,s_j}}{\partial t}\\
  %  &=-d_{ij}\cdot x^{OPT}_{ij}\cdot \frac{\frac{\partial x_{ij}}{\partial t}}{x_{ij} %+ \frac{x^{OPT}_{ij}}{k} } - o_j\cdot \frac{2^{s_j}}{m}\cdot \frac{\frac{\partial %y_{j}}{\partial t}}{y_{j}+\frac{2^{s_j-1}}{mk}}\\
  %  &=-\frac{d_{ij}}{d_{ij}+o_j}\cdot x^{OPT}_{ij} \cdot \left(\frac{x_{ij} + %\frac{\Gamma_{ij}}{k}}{x_{ij} + \frac{x^{OPT}_{ij}}{k}}\right) - %\frac{o_j}{d_{ij}+o_j}\cdot \frac{2^{s_j}}{m} \cdot \left(\frac{x_{ij} + %\frac{\Gamma_{ij}}{k}}{x_{ij} + \frac{2^{s_j-1}}{mk}}\right)\\
  %  &\le -\frac{d_{ij}}{d_{ij}+o_j}\cdot x^{OPT}_{ij}  - \frac{o_j}{d_{ij}+o_j}\cdot %\frac{2^{s_j}}{m}\text{. (Since $\Gamma_{ij} \ge x^{OPT}_{ij} \ge %\frac{2^{s_j-1}}{m}$)}\\
  %  &\le -x^{OPT}_{ij},
%\end{align*}
%
%\end{proof}


We now combine these lemmas to show the following result:
\begin{proof}
    Initially, let $x_{ij} = y_j = 0$ for all $i, j$ but let $\xd_{ij}, \yd_j$ be their final value. 
    %(Note that the algorithm doesn't set the values of $\xd_i$, in fact it doesn't even know the values -- this is just for bounding the cost in the analysis.) 
    Then, by \Cref{lem:opt-pot1}, the potential $\phi$ is at most $O(\log k)$ times the cost of \dynamic. Now, as \Cref{alg: Dynamic_OPT_fac_loc} increases the values of the variables $x_{ij}, y_j$, it incurs cost at rate at most $\frac32$ (by \Cref{lem:costfac}) and the potential $\phi$ decreases at rate at least $\frac12$ (by \Cref{lem:alg-pot1}). Since $\phi$ is always non-negative (by \Cref{lem:pot-nonneg1}), it follows that the total cost of the algorithm is at most $3$ times the potential $\phi$ at the beginning, i.e., at most $O(\log k)$ times the \dynamic benchmark. 
\end{proof}

We also note that \Cref{thm:fracfl} cannot be improved further (except lower order terms) without improving the best online algorithm (without prediction) for facility location. This is because the best known online fractional algorithm for the problem obtains a competitive ratio of $\tilde{O}(\log n)$ where $n$ is the number of clients. This is even if the client locations and potential facility locations are identical, in which we can simulate an instance of the online facility location problem without predictions by giving all prior client locations as suggested facility locations (for $k=n$). Furthermore, it is known (see Meyerson~\cite{Meyerson01}) that there is no $O(1)$-competitive algorithm for the online facility location problem, and this lower bound construction easily extends to the fractional version of the problem.
